Evaluation of synthetic and experimental training data in supervised machine learning applied to charge state detection of quantum dots

Automated tuning of gate-defined quantum dots is a requirement for large scale semiconductor based qubit initialisation. An essential step of these tuning procedures is charge state detection based on charge stability diagrams. Using supervised machine learning to perform this task requires a large dataset for models to train on. In order to avoid hand labelling experimental data, synthetic data has been explored as an alternative. While providing a significant increase in the size of the training dataset compared to using experimental data, using synthetic data means that classifiers are trained on data sourced from a different distribution than the experimental data that is part of the tuning process. Here we evaluate the prediction accuracy of a range of machine learning models trained on simulated and experimental data and their ability to generalise to experimental charge stability diagrams in two dimensional electron gas and nanowire devices. We find that classifiers perform best on either purely experimental or a combination of synthetic and experimental training data, and that adding common experimental noise signatures to the synthetic data does not dramatically improve the classification accuracy. These results suggest that experimental training data as well as realistic quantum dot simulations and noise models are essential in charge state detection using supervised machine learning.

==> tables/KNeighborsClassifier_test_score.tex <==
\begin{tabular}{@{\extracolsep{8pt}}lccccc}
\hline \hline 
\multicolumn{6}{c}{KNeighborsClassifier}  \\ \cline{1-6} 

\hline \hline
\end{tabular}


==> tables/my_CNN_acc.tex <==
\begin{tabular}{@{\extracolsep{6pt}}lccccc}
\hline \hline
    train acc &                                          synthetic &                                          clean exp &                                           good exp &                                            all exp \\
\hline
 99.22 (0.59) &  {'conf_mat': '$egin{bmatrix} 1048.43 (20.89) ... &  {'conf_mat': '$egin{bmatrix} 90.29 (4.46) & 1... &  {'conf_mat': '$egin{bmatrix} 405.90 (38.28) &... &  {'conf_mat': '$egin{bmatrix} 722.00 (101.12) ... \\
 97.52 (1.61) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix} 88.38 (6.61) & 1... &  {'conf_mat': '$egin{bmatrix} 366.22 (42.14) &... &  {'conf_mat': '$egin{bmatrix} 601.40 (114.09) ... \\
 90.57 (5.02) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix} 96.17 (2.27) & 5... &  {'conf_mat': '$egin{bmatrix} 90.20 (6.91) & 1... &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... \\
 91.28 (4.63) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... &  {'conf_mat': '$egin{bmatrix} 169.80 (11.09) &... \\
\hline \hline
\end{tabular}


==> tables/noise_stats_my_CNN_conf_mat.tex <==
\begin{tabular}{@{\extracolsep{8pt}}lcccc} 
 \hline \hline 
 & \multicolumn{4}{c}{accuracy}  \\ \cline{2-5} 
max noise amplitude  & training & clean experimental & good experimental & all experimental \\
\hline \multicolumn{5}{c}{white} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                               good experimental &                                all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $\begin{bmatrix}93&8\\11&90\end{bmatrix}$ &  $\begin{bmatrix}382&166\\148&401\end{bmatrix}$ &  $\begin{bmatrix}594&503\\304&794\end{bmatrix}$ \\

\hline  \hline 
\multicolumn{5}{c}{random telegraph} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                          good experimental &                           all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.1  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.2  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.3  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\

\hline  \hline 
\multicolumn{5}{c}{random current modulation} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                          good experimental &                           all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.1  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.2  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.3  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\

\hline  \hline 
\multicolumn{5}{c}{pinchoff modulation} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                          good experimental &                           all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.1  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.2  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.3  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\

\hline  \hline 
\multicolumn{5}{c}{1/f} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                          good experimental &                           all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.1  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.2  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.3  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\

\hline  \hline 
\multicolumn{5}{c}{charge jumps} \\ \cline{1-5}{}

{} &                                   training &                         clean experimental &                          good experimental &                           all experimental \\

0.05 &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.1  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.2  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\
0.3  &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ &  $ \begin{bmatrix}  & \\ & \end{bmatrix} $ \\

\hline  \hline 
\hline \hline
 \end{tabular}


==> tables/noise_stats_qf_CNN_conf_mat.tex <==
\begin{tabular}{@{\extracolsep{8pt}}lcccc} 
 \hline \hline 
 & \multicolumn{4}{c}{accuracy}  \\ \cline{2-5} 
max noise amplitude  & training & clean experimental & good experimental & all experimental \\
\hline \hline \hline
 \end{tabular}


==> tables/noise_stats_qf_CNN_test_score.tex <==
\begin{tabular}{@{\extracolsep{8pt}}lcccc} 
 \hline \hline 
 & \multicolumn{4}{c}{accuracy}  \\ \cline{2-5} 
max noise amplitude  & training & clean experimental & good experimental & all experimental \\
\hline \multicolumn{5}{c}{No noise} \\ \cline{1-5} {}

 
0 &  99.64 (0.16) &       77.19 (3.49) &      64.43 (1.99) &     61.74 (1.57) \\

\hline  \hline 
\hline \hline
 \end{tabular}


==> tables/qf_CNN_acc.tex <==
\begin{tabular}{@{\extracolsep{6pt}}lccccc}
\hline \hline
    train acc &                                          synthetic &                                          clean exp &                                           good exp &                                            all exp \\
\hline
 99.64 (0.16) &  {'conf_mat': '$egin{bmatrix} 1046.67 (15.47) ... &  {'conf_mat': '$egin{bmatrix} 68.67 (9.68) & 3... &  {'conf_mat': '$egin{bmatrix} 323.25 (52.60) &... &  {'conf_mat': '$egin{bmatrix} 699.41 (104.09) ... \\
 98.65 (1.10) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix} 60.86 (5.74) & 4... &  {'conf_mat': '$egin{bmatrix} 303.90 (39.00) &... &  {'conf_mat': '$egin{bmatrix} 623.70 (87.46) &... \\
 91.30 (4.82) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... &  {'conf_mat': '$egin{bmatrix} 87.36 (9.43) & 2... &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... \\
 90.61 (3.24) &                              {'conf_mat': '- (-)'} &  {'conf_mat': '$egin{bmatrix} 85.67 (7.99) & 1... &  {'conf_mat': '$egin{bmatrix}  & \ & \end{bmat... &  {'conf_mat': '$egin{bmatrix} 173.80 (6.91) & ... \\
\hline \hline
\end{tabular}


==> tables/qf_CNN_conf_mat.tex <==
\begin{tabular}{@{\extracolsep{8pt}}lccccc}
\hline \hline 
  training data & \multicolumn{5}{c}{average accuracy (std)}  \\ \cline{2-6} 

{} &      training &                                       synthetic &                          clean experimental &                               good experimental &                                all experimental \\
\hline
synthetic                       &  99.64 (0.16) &  $\begin{bmatrix}1043&56\\33&1052\end{bmatrix}$ &  $\begin{bmatrix}68&33\\14&87\end{bmatrix}$ &  $\begin{bmatrix}323&225\\165&383\end{bmatrix}$ &  $\begin{bmatrix}699&398\\440&657\end{bmatrix}$ \\
good experimental               &  91.30 (4.82) &                                           - (-) &  $\begin{bmatrix}88&13\\22&79\end{bmatrix}$ &      $\begin{bmatrix}87&21\\29&81\end{bmatrix}$ &    $\begin{bmatrix}167&50\\80&142\end{bmatrix}$ \\
all experimental                &  90.61 (3.24) &                                           - (-) &  $\begin{bmatrix}85&16\\18&83\end{bmatrix}$ &      $\begin{bmatrix}81&30\\24&83\end{bmatrix}$ &    $\begin{bmatrix}171&50\\70&147\end{bmatrix}$ \\
synthetic and good experimental &  98.29 (1.13) &                                           - (-) &   $\begin{bmatrix}93&8\\13&88\end{bmatrix}$ &      $\begin{bmatrix}96&16\\31&75\end{bmatrix}$ &    $\begin{bmatrix}181&41\\92&124\end{bmatrix}$ \\
synthetic and all experimental  &  96.99 (1.61) &                                           - (-) &  $\begin{bmatrix}91&10\\12&89\end{bmatrix}$ &      $\begin{bmatrix}87&22\\25&84\end{bmatrix}$ &    $\begin{bmatrix}166&53\\64&155\end{bmatrix}$ \\
synthetic with noise            &  98.65 (1.10) &                                           - (-) &  $\begin{bmatrix}61&40\\10&91\end{bmatrix}$ &  $\begin{bmatrix}303&245\\147&401\end{bmatrix}$ &  $\begin{bmatrix}623&474\\382&716\end{bmatrix}$ \\
\hline \hline
\end{tabular}

